Graph Embeddings at Scale

Graph embedding is a popular algorithmic approach for creating vector representations for individual vertices in networks. Training these algorithms at scale is important for creating embeddings that can be used for classification, ranking, recommendation and other common applications in industry. While industrial systems exist for training graph embeddings on large datasets, many of these distributed architectures are forced to partition copious amounts of data and model logic across many worker nodes. In this paper, we propose a distributed infrastructure that completely avoids graph partitioning, dynamically creates size constrained computational graphs across worker nodes, and uses highly efficient indexing operations for updating embeddings that allow the system to function at scale. We show that our system can scale an existing embeddings algorithm - skip-gram - to train on the open-source Friendster network (68 million vertices) and on an internal heterogeneous graph (50 million vertices). We measure the performance of our system on two key quantitative metrics: link-prediction accuracy and rate of convergence. We conclude this work by analyzing how a greater number of worker nodes actually improves our system's performance on the aforementioned metrics and discuss our next steps for rigorously evaluating the embedding vectors produced by our system.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
		Corrected the bug with acmPrice.
		Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
		The package now is compatible with polyglossia (Joachim Breitner).
		Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
		Deleted indent for subsubsection (suggested by Ross Moore)
		Suppressed some obscurious warning in BibTeX processing
		Suppressed hyperrerf warnings (Paolo G. Giarrusso)
		New code for sections to help with accessibility patches
		(Ross Moore)
		Submission id, if present, is printed in anon mode
		Bug fixes

Version 1.55    Bug fixes


==> embeddings_body.tex <==
\section{Introduction}
\todo{Re-approach this \& the abstract at the very end.}
Graph embeddings, how they work, how they are trained and what they can be used to do

Two types of scale: size (number of edges) and order (number of nodes). These are inherent properties of graphs, whereas in language modeling the 'size' corresponds to number of unique vocabulary words and the 'order' is a function of the size of the corpus and the context window size. 

% Compute - CPU/GPU
% Network
% Memory

% How others have approached this challenge

% Our contribution

% Experiments we run

% Results we have found


\section{Related Work}
While neural embedding models have effectively created rich mathematical representations for words in natural language processing, attempting to model relationships between entities in larger industrial systems - such as the links between users in a social network graph - require a far more scalable approach. For example, complex recommendation engines typically compare millions of users with items, which is commonly modeled as a relationship graph that might contain billions of edges between these two entities. Consequently, graph embedding techniques have been recently used in a few modern systems to create meaningful relationships between entities even in such a large graph. 

In this section, we will examine how both algorithmic and infrastructural advancements have benefited the training of large-scale distributed models. Several of the systems in this section particularly formulate problems with graph embeddings and advanced parameter updating frameworks.

\subsection{Algorithmic Advancements with Large-Scale Embedding Systems}

\subsubsection{Pinterest's Pixie Recommendation Engine:}
Many recommendation systems that use techniques from graph theory first impose a graph-like structure on an existing dataset and then run random walk algorithms to compare the importance of individual nodes to one another. For example, Pinterest's Pixie Recommendation system relates billions of edges between "pins" and "boards" with an undirected bipartite graph. However, Pixie only ever interacts with subsets of this graph by looking at a time window of a user's most recently submitted queries - for specific pins or boards - and then runs random walks starting from these visited entities to find the most relevant content for a user. Pixie also biases its random walks in a user-specific way: the systems weights edges differently from one another depending on the user's own preferences on Pinterest.

While Pixie uses a clever technique to find relevant content for its users, the system relies on a few key assumptions that might hinder its efficiency on other graph-based problems. Firstly, Pixie prunes boards and its respective edges from the main relationship graph if the former entity has a high entropy distribution of pin variety. However, the system must use external annotations - such as captions and descriptions - to compute the content diversity of its entities, and this requirement limits its generalizability to other large-scale industrial problems that might not have text or visual accompaniment. Pixie's graph pruning approach is also likely how the system is able to store an entire graph on a single worker node in a distributed training job. However, systems with similarly-sized graphs that cannot prune based off external information would likely need to partition their graph across several nodes, which can heavily impact inference speed if a query must require multiple partitions to complete a random walk, and prediction quality if many untrimmed edges add noise to existing relationships in a graph.  

\subsubsection{Alibaba's Billion-Scale Item Embeddings:}
 Another interesting case study of large-scale embedding models is the Base Embeddings System (BES) model at Alibaba, where researchers train a graph embedding model on a billion-scale item-to-item graph network to recommend products for consumers in Alibaba's Taobao E-Commerice platform. Unlike the bipartite relationship graph at Pinterest, the BES system constructs a directed graph that connects billions of items with one another based off user behavior on Alibaba's platform. Researchers then run DeepWalk, a graph-based algorithm inspired by Word2Vec, on this network to learn the latent representations for each item in their catalogue. 

Alibaba's system takes advantage of a key insight in the structure of their data; items that are closely related to one another are frequently at one edge length in distance across all user sessions. Taking this sequential purchase information into account underscores the effectiveness of a graph-based approach over a more traditional recommendation engine method (e.g collaborative filtering) that might only rely on the co-occurrence of different items to assess their similarity. Alibaba's graph embeddings model also incorporate external data, or "side information" vectors, that boosts the quality of item embeddings that might have few connections to other products on their platforms. Unlike the text and visual annotations that are used in Pinterest's Pixie system, these side information vectors represent more abstract entities - category, price, or brand type - which makes Alibaba's approach better generalizable to other large-scale industrial systems that need to derive information from an abstract entity relationship graph. 

While Alibaba's BES system is able to construct high-quality item embeddings in a production environment, the graph network itself is too large to store on any single machine in their distributed Open Data Processing Service (ODPS) network. This is partly because Alibaba's graph embeddings models use an adjacency matrix to represent edge links between items. Unlike in Pinterest's Pixie system, this is a memory exhaustive approach and is likely why their item-to-item network must be partitioned across several subgraphs for effective usage. Consequently, this prevents data replication across worker nodes and could hamper the availability of their distributed system in the case of node failure. A more efficient system that can combine the generalizability of Alibaba's graph embeddings approach and Pixie's efficient graph storage setup would be a desirable solution for maintaining scalability with high performance on any entity-to-entity relationship graph.

\subsection{Infrastructural Advancements with Large-Scale Embedding Systems}

Along with optimizing for algorithmic effectiveness with a graph embeddings framework, an efficient infrastructure is also required for training any production-ready system. Prior to recent advancements in distributed training today, most production systems relied on simpler distributed data-parallel systems like Apache Spark MLLib or Deeplearning4j to train millions of different embedding vectors. However, forcing Spark executors to store local copies of a global embeddings lookup table is not scalable for vocabularies that are millions of entities large, which is typical for problems outside of the NLP space. Today, the most well-known distributed architecture for training very large machine learning models relies on a centralized parameter server to store a global list of parameters during the course of training. 

\subsubsection{Yahoo's Distributed Training of Large Word2Vec Systems:}

While a parameter server has been effectively applied to the training of very large models for logistic regression, deep learning, and factorization machines, this method typically require too much network bandwidth for acceptable training throughput. Researchers at Yahoo Labs  recently developed a distributed Word2Vec training system for the purpose of matching millions of queries to ads in their Gemini platform. Their system proposes a columnar partitioning approach that assigns columns from embedding vectors to different parameter server shards - for example, a vector dimension d = 300 that is columnar partitioned equally into 20 parameter server shards would hold 30 embedding components each. Consequently, for $S$ parameter shards, their system is able to scale up vocabulary size by a factor of $S$ relative to training on a single machine. 

Vertically partitioning these embedding vectors can arguably decrease network bandwidth ensued while retrieving and updating them from a global server. However, the maximum embedding dimension size in current literature is already capped around 500, whereas the number of embeddings itself is extremely variable depending on the application. Thus, systems with smaller dimensional requirements might not strongly benefit from the columnar partitioning approach that is proposed by the authors. Instead, horizontally partitioning an embeddings lookup table would likely be more effective for training large-scale systems that store embedding vectors to represent millions of different samples. The system proposed in this paper uniquely tackles this problem by using a modification of the parameter server approach to adequately store store data and parameters across worker nodes in a distributed setting without suffering from excessive network bandwidth costs. 


\subsubsection{HogWild! Asynchronous Training of Large-Scale Datasets:}
One challenge from using stochastic gradient descent (SGD) is parallelizing gradient updates from several points of data during training. This algorithm is inherently serial and training on a large-scale dataset may take an inordinate amount of time if implemented in a non-distributed fashion. Prior to advancements with asynchronous distributed training, most of the best approaches for speeding up serial algorithms required using additional computational power (e.g, GPUs) to iterate a model on larger batches of training data. Locking mechanisms were also explored for parallelizing SGD but failed to drastically reduce training time because synchronization adds significant time delay; for example, while an update step might take on the order of microseconds, acquiring a lock and releasing it can take a few milliseconds. A change on this order of magnitude makes locking nearly 1000x longer to execute than updating a model's parameters.

$HogWild!$ proposes asynchronous training of large-scale datasets without any synchronization. Thus, all threads on a multi-core system should read and write to a global list of model parameters at any time during a training job. Part of $HogWild!'s$ success comes from its proof that asynchronous training has zero negative impact on the rate of convergence for a large-scale machine learning model, which has been successfully extended to many different applications (e.g stochastic coordinate descent for SVMs, randomized Kaczmarz algorithms for solving systems of linear equations) in current literature. We partly attribute the success of our own distributed architecture from adopting the $HogWild!$ philosophy while training graph embedding models on the large-scale datasets in this paper. 

\section{Proposed Approach}
Embedding a graph in dense vector space is often accomplished by joining two components: a random walk algorithm and a neural embedding model \cite{DBLP:journals/corr/GroverL16, DBLP:journals/corr/PerozziAS14}. The random walk algorithm can take a variety of forms and constraints but generally speaking it is used to define a training set for the neural embedding model. This training set comprises a series of examples of vertices that should be similar in the embedding space and often includes examples of vertices that should be dissimilar.  From an infrastructure perspective we take a decoupled approach, first generating the sequence as a training dataset followed by learning on the sequences themselves. This allows us to utilize the significant performance enhancements that have already been established for random walk algorithmic implementations.  At the same time, it allows us to focus on solving the various constraints of scaling neural embedding models to billions of nodes.

\subsection{Graph Walk Algorithms}
Although our approach allows for a variety of graph walk algorithms a few things should be noted about how to use these. Firstly, some other approaches have proposed graph partitioning \cite{wang2018billion} as a means of constraining the number of nodes per worker and allowing for parallelization. The benefits of this is that each worker can get a distinct subset of nodes and therefore no centralized parameter store or synchronization. If there are no existing subgraphs then partitioning has to occur by severing edges. Accomplishing a balanced partition that minimizes the edges cut is an NP-hard problem \cite{Tsourakakis:2014:FSG:2556195.2556213}. While approximations exist, if possible we find it better to use other mechanisms for parallelizing the training of this model that don't involve partitioning the graph. For example, approaches such as those described in Eksombatchai, et. al. \cite{eksombatchai2018pixie} allow for the graph algorithmic portion of the embedding model to be performed in memory on a single node even on very large (3 billion node) graphs.

Secondly, we constrain our graph walk algorithm to have small context window, essentially only modeling first order relationships between vertices. The motivation here is to guarantee true noise samples. If context is defined as a shared edge than for any vertex any non-edge becomes a valid noise sample. If context is defined, as it is in DeepWalk, of five steps on the graph then it becomes to hard to guarantee that a randomly generated noise vertex won't appear within five steps of that given node. Depending on the graph at a certain context size everything becomes related and the idea of noise sampling becomes irrelevant.

The number of training pairs generated by a graph walk algorithm as a function of walk length (l), context window (c) and walks per node (w) is:

\begin{math}
  pairs = w*\sum_{j=2}^{c} (l-j+1)
\end{math}

If we constrain c=2 then this reduces to:

\begin{math}
  pairs = w*(l-1)
\end{math}

With that constraint in place any reduction in walk length can then be offset by taking more walks per node. This can be seen in figure 1. Here we take a graph of unique prime integers (0, 1, 2, 3) and plot the distribution of edges comprised of multiplying those values. As can be seen, when the window size is fixed (two), there is little difference in recovering the distribution of edges as a function of walk length and number of walks per node.

\begin{figure}
\includegraphics[width=4cm,
                 keepaspectratio,]{figures/10_short_walks.png}
\includegraphics[width=4cm,
                 keepaspectratio,]{figures/10_long_walks.png}
\includegraphics[width=4cm,
                 keepaspectratio,]{figures/80_short_walks.png}
\includegraphics[width=4cm,
                 keepaspectratio,]{figures/80_long_walks.png}
\caption{Edge distributions with a) ten walks of length two b) ten walks of length eighty c) eighty walks of length two d) eighty walks of length eighty}
\end{figure}


\subsection{Distributed training}
For any sufficiently large graph, the number of training pairs generated by a graph walk algorithm will far exceed what is computationally tractable on a single machine. At the same time it can be observed that a limited number of nodes appear on any given subset of training data. Thus, parallelization can be achieved by splitting the training set across a number of workers that execute in parallel asynchronously and unaware of the existence of each other. Each worker loads a batch of data, trains and updates the embeddings of nodes appearing in this batch only. Distributed training relies on a centralized parameter repository that allows learning to be shared across all the workers. In the case of graph embeddings, a parameter server can hold the embeddings table which contains the vectors corresponding to each node in the graph. The embeddings table is a $N x D$ table, where $N$ is the number of nodes in the graph and $D$ is a hyperparameter that denotes the number of embedding dimensions. The parameter servers utilize row based index id where the id of a node equals the row id in the table. This allows for highly efficient retrievals and updates.

On each training iteration, the workers load a subset (batch) of training data which can contain a variable number of unique nodes. The embeddings of these unique nodes are requested from the parameter server. Because embedding lookup functions in the Tensorflow require the data to be formatted as an index referencing its location in a Tensor (of maximum size 2GB) a mapping is created from the parameter server index to the worker's tensor index. After training takes place on the worker, the embeddings are updated on the parameter server. The proposed architecture is depicted in Figure \ref{arch_fig}. Each worker executes the following steps:

\begin{algorithmic}
\STATE Determine size of training subset
\STATE $dataSize\gets nSteps * batchSize$
\FOR{iter in size(trainingData) / dataSize}
    \STATE $subset\gets trainingData / dataSize$
    \STATE $uniqueNodes\gets set(subset)$
    \STATE $localIdx\gets 0$
    \FOR{node in uniqueNodes} 
        \STATE $nodeToLocal[node]\gets localIdx$
        \STATE $localToNode[localIdx]\gets node$
        \STATE $localIdx \gets localIdx + 1$
    \ENDFOR
    \STATE Replace ids in subset of data with local indices
    \FOR{row in subset}
        \FOR{element in row}
            \STATE $localElement\gets nodeToLocal[element]$
        \ENDFOR
    \ENDFOR
    \STATE Request existing embeddings from server for unique nodes
    \STATE $initialEmbeddings\gets serverRequest(uniqueNodes)$
    \STATE Uses these embeddings as intializations for embeddings tensor in graph
    \STATE $embeddingsTensor\gets initialEmbeddings$
    \FOR{step in nSteps}
        \STATE Train embeddings using batch of subset data
    \ENDFOR
    \STATE Map rows in embeddings tensor back to global values
    \STATE Send trained embeddings back to server to update values
\ENDFOR
\end{algorithmic}

\begin{figure}
\includegraphics[width=4cm,
                 keepaspectratio,]{figures/ColumnarPartition.png}
\includegraphics[width=4cm,
                 keepaspectratio,]{figures/row_partition.png}
\caption{Memory requirements for a) columnar partition and b) row-wise partition}
\end{figure}

This system of training is fully asynchronous without locking as used in Recht, et. al. \cite{recht2011hogwild}. The same assumptions made in that framework is that any two subsets of data will have a limited number of shared nodes and therefore update conflicts will be limited. If there is a collision then the server request that came latest will overwrite the previous update before any other request can use them in training. Over large datasets we expect this to have minimal impact. Another possibility is that while one worker is updating the embedding of a node another worker requests that embedding and gets some portion of the older vector and some portion of the one being written. Because the gradients are small between training iterations the difference between the last version the embedding and the updated version should also be limited.

\begin{figure}
\includegraphics[width=8cm, keepaspectratio,]{figures/arch.png}
\label{arch_fig}
\caption{Distributed training architecture diagram}
\end{figure}

\subsection{Parameter server partitioning}
In a typical graph embedding scenario, $D$ can be set anywhere from 100 - 300.  In very large graphs (nodes > 1 Billion), the memory requirements of serving these embeddings can quickly exceed what can be done by commodity servers. Therefore partitioning strategies must be employed which commonly either partition across the rows (nodes) or the columns (embedding dimensions) of the table. Column wise partitioning, as laid out in \cite{grbovic2015commerce}, maintains a number of columns for every node on each parameter server. This achieves good load balancing as every server is queried once by each worker on each training iteration. The disadvantage is that it restricts the maximum number of parameter servers to the number of embedding dimensions. At the same time, it must be ensured that at a minimum, a single column can fit into the memory of every parameter server.

On the other hand, partitioning the embedding table row-wise does not impose any restrictions. Each parameter server holds all the embedding dimensions for a number of nodes. The disadvantage is that parameter servers that hold the embeddings for nodes that appear more often in the training pairs will receive a high number of requests. This can be addressed by utilizing a bin packing approach where the nodes are distributed across the servers in accordance to server capacity and the number of times each node appears in the training pairs. Bin packing is an NP-hard problem, thus heuristic solutions are used. In our approach, we implement column wise partitioning unless the size of a single column exceeds the capacity of any server in which case we revert to row wise partitioning. In both approaches, no effort has been made to implement server fault tolerance and the number of servers, graph nodes and training pairs are expected to remain static during training.
% Row based indexing of nodes, the ID of the node is the row ID in the embedding table. This allows for efficient lookups. 

%The training data contains the node index ids corresponding to the row in the parameter server. 





% On each iteration, a subset of data is loaded. This subset of data is then divided into training batches. subsets of data can contain variable numbers of nodes.




%However, the embedding lookup function requires an index into a table in the tensor computational graph on the worker. 





% Batching within worker
% Utilization of GPUs, while speeding up computation, introduces an additional constraint in GPU memory. Many common neural network training frameworks such as Tensorflow \cite{abadi2016tensorflow}, impose a limit of 2GB on any given tensor in your computational graph. This means that for any embedding dimension \begin{math}d\end{math}, the maximum number of nodes \begin{math}n\end{math} can be determined by \begin{math}n = 2e^9 / (4 * d) \end{math} assuming that your embedding vectors are float32 (4 bytes).  Therefore, to accommodate the GPU memory constraint each worker only loads in a subset data that reasonably won't have more nodes than the 2GB limit would allow. 
 

 
% This subset of data is then divided into training batches. Because the graph is not partitioned in advance, and because negative sampling is computed dynamically and on the entire embedding space, subsets of data can contain variable numbers of nodes.

% Therefore, a new computational graph needs to be initiated to correspond exactly to the tensor size of each subset. 

% network traffic increases but it is theoretically only limited by the number of provisionable parameter servers.  This relationship can be seen in Figure 2.

% In the case of this approach the embedding space is partitioned by nodes. The nodes are divided into p shards and each embedding server contains a single shard.  

%a single column does not fit, shard size, column wise is the advantageous approach.
% However, at the next level of scale you are constrained by the number of embedding dimensions. A standard embedding size is 128, this means that you cannot partition your graph beyond 128 servers. 
% It should be acknowledged that in practice, using commodity hardware with 128 gb of RAM it would take a graph of four trillion nodes to reach the limit of columnar based partitioning.



% If network bandwidth is a constraint then it may be best to use a columnar-style approach. In the intermediate scales this also accomplishes a scalability with regards to the number of graph nodes you can hold in your parameter store. 








 








% \subsection{Partitioning Parameter Server}
% Most distributed training systems rely in some form on a centralized parameter server. This parameter server allows learning to be shared across all the workers. In the case of graph embeddings the parameter server holds the vectors corresponding to each node in the graph. In a typical graph embedding the dimensions of these embeddings, a hyperparameter, can be set anywhere from 100 - 300.  In very large graphs (nodes > 1 Billion), the memory requirements of serving these embeddings can quickly exceed what can be done by commodity infrastructure. Therefore partitioning strategies must be employed. In the case of this approach the embedding space is partitioned by nodes. The nodes are divided into p shards and each embedding server contains a single shard.  

% \textcolor{red}{Thanos describe the numpy indexing thing here}

% \begin{figure}
% \includegraphics[width=4cm,
%                  keepaspectratio,]{ColumnarPartition.png}
% \includegraphics[width=4cm,
%                  keepaspectratio,]{row_partition.png}
% \caption{Memory requirements for a) columnar partition and b) row-wise partition}
% \end{figure}

% If network bandwidth is a constraint then it may be best to use a columnar-style approach as laid out in \cite{grbovic2015commerce}. In the intermediate scales this also accomplishes a scalability with regards to the number of graph nodes you can hold in your parameter store. However, at the next level of scale you are constrained by the number of embedding dimensions. A standard embedding size is 128, this means that you cannot partition your graph beyond 128 servers. On the other hand, in our approach, partitioning the embedding table row-wise (e.g. by nodes in the graph), network traffic increases but it is theoretically only limited by the number of provisionable parameter servers. It should be acknowledged that in practice, using commodity hardware with 128 gb of RAM it would take a graph of four trillion nodes to reach the limit of columnar based partitioning. This relationship can be seen in Figure 2.

% \subsection{Dynamic Memory Bound Computational Graphs}
% Utilization of GPUs, while speeding up computation, introduces an additional constraint in GPU memory. Many common neural network training frameworks such as Tensorflow \cite{abadi2016tensorflow}, impose a limit of 2GB on any given tensor in your computational graph. This means that for any embedding dimension \begin{math}d\end{math}, the maximum number of nodes \begin{math}n\end{math} can be determined by \begin{math}n = 2e^9 / (4 * d) \end{math} assuming that your embedding vectors are float32 (4 bytes). At the same time it can be observed that for any given subset of training data there will be a limited number of nodes that appear. Therefore, to accommodate the GPU memory constraint each worker only loads in a subset data that reasonably won't have more nodes than the 2GB limit would allow. This subset of data is then divided into training batches. Because the graph is not partitioned in advance, and because negative sampling is computed dynamically and on the entire embedding space, subsets of data can contain variable numbers of nodes. Therefore, a new computational graph needs to be initiated to correspond exactly to the tensor size of each subset. The training data contains the index ids corresponding to the row in the parameter server. However, the embedding lookup function requires an index into a table in the tensor computational graph on the worker. It is necessary then to create a mapping from the parameter server index to the worker index. Each worker, in parallel, completes the training iteration following the steps below

% \begin{algorithmic}
% \STATE Determine size of training subset
% \STATE $dataSize\gets nSteps * batchSize$
% \FOR{iter in size(trainingData) / dataSize}
%     \STATE $subset\gets trainingData / dataSize$
%     \STATE $uniqueNodes\gets set(subset)$
%     \STATE $localIdx\gets 0$
%     \FOR{node in uniqueNodes} 
%         \STATE $nodeToLocal[node]\gets localIdx$
%         \STATE $localToNode[localIdx]\gets node$
%         \STATE $localIdx \gets localIdx + 1$
%     \ENDFOR
%     \STATE Replace ids in subset of data with local indices
%     \FOR{row in subset}
%         \FOR{element in row}
%             \STATE $localElement\gets nodeToLocal[element]$
%         \ENDFOR
%     \ENDFOR
%     \STATE Request existing embeddings from server for unique nodes
%     \STATE $initialEmbeddings\gets serverRequest(uniqueNodes)$
%     \STATE Uses these embeddings as intializations for embeddings tensor in graph
%     \STATE $embeddingsTensor\gets initialEmbeddings$
%     \FOR{step in nSteps}
%         \STATE Train embeddings using batch of subset data
%     \ENDFOR
%     \STATE Map rows in embeddings tensor back to global values
%     \STATE Send trained embeddings back to server to update values
% \ENDFOR
% \end{algorithmic}

% This system of training is fully asynchronous without locking as used in Recht, et. al. \cite{recht2011hogwild}. The same assumptions made in that framework is that any two subsets of data will have a limited number of shared nodes and therefore update conflicts will be limited. If there is a collision then the server request that came latest will overwrite the previous update before any other request can use them in training. Over large datasets we expect this to have minimal impact. Another possibility is that while one worker is updating the embedding of a node another worker requests that embedding and gets some portion of the older vector and some portion of the one being written. Because the gradients are small between training iterations the difference between the last version the embedding and the updated version should be limited.

\subsection{Softmax Approximations}

The standard neural embedding model used is the skip-gram word2vec model. The word2vec model words are embedded in dense vector space by sliding a window over sequences of words in a corpus. For each word the task then becomes using the vector representation of each word to predict the words immediately before and after it in the window  \cite{NIPS2013_5021}.  While the exact formulation for this task requires an expensive computation of a softmax over all possible vocabulary words, two approximations have gained prominence in practice: hierarchical softmax and noise contrastive estimation (NCE) \cite{mnih2013learning, DBLP:journals/corr/cs-CL-0108006}. 

NCE was first proposed by Gutman et. al. \cite{pmlr-v9-gutmann10a} and then applied to word embeddings by Mnih et. al. \cite{mnih2013learning} has gained equal popularity to the hierarchical softmax as an approximation of the softmax. NCE decomposes the skip-gram algorithm into a binary classification task. In this task for an input word x, observed context words Y and a set of randomly generated noise samples N, the model fits a logistic regression model to the embedding layer such that it can distinguish between the noise samples N and the true context words Y when given x.

This model has been further generalized by observing simplifying the logistic regression task. This is accomplished by directly comparing the vectors of the input word x, context word y and noise samples N in a pairwise fashion. The choice of comparison function can vary, but frequently is cosine similarity or another distance metric. When generalized beyond language, the objective of this model is to determine a low dimensional representation of an vertex in a graph such that its distance to observed edges on the graph in the low dimension space is minimized while maximizing its distance from observed non-edges  \cite{DBLP:journals/corr/abs-1709-03856}. This objective has been shown to be factorizing the adjacency matrix \cite{TACL570}. However, because it explicitly models non-edges in the noise sampling procedure it captures relationships that matrix factorization cannot. 

Finally, for the purpose of the architecture in question, the generalized noise contrastive estimation framework as laid out in Wu et. al. has performance advantages over both hierarchical softmax and traditional noise contrastive estimation. In the case of the former, it is required that during training the entirety of the binary search tree is maintained by the neural network. In a distributed training paradigm this would be computationally efficient but not memory efficient \textcolor{red}{Is this accurate??}. On the other hand, NCE can be very memory efficient, at each step in training the model really only needs the vectors and weights corresponding specifically to the vertices in the training batch. As will be shown further on in this paper, this property allows for significant parallelization. Furthermore, by using the simpler NCE with just the distance metrics, the memory footprint of the model is halved. 

% \subsection{Architecture}

% \textcolor{red}{Include architectural diagrams??}


\section{Experiments}
Detailed description

\subsection{Dataset}

\subsection{Results}

\section{Conclusions}
You know. what we learned

\appendix
%Appendix A
Here is an outline of the body of this
document in Appendix-appropriate form:
\subsection{Introduction}
\subsection{The Body of the Paper}
\subsubsection{Type Changes and  Special Characters}
\subsubsection{Math Equations}
\paragraph{Inline (In-text) Equations}
\paragraph{Display Equations}
\subsubsection{Citations}
\subsubsection{Tables}
\subsubsection{Figures}
\subsubsection{Theorem-like Constructs}
\subsubsection*{A Caveat for the \TeX\ Expert}
\subsection{Conclusions}
\subsection{References}
Generated by bibtex from your \texttt{.bib} file.  Run latex,
then bibtex, then latex twice (to resolve references)
to create the \texttt{.bbl} file.  Insert that \texttt{.bbl}
file into the \texttt{.tex} source file and comment out
the command \texttt{{\char'134}thebibliography}.
% This next section command marks the start of
% % Appendix B, and does not continue the present hierarchy
% \section{More Help for the Hardy}

% Of course, reading the source code is always useful.  The file
% \path{acmart.pdf} contains both the user guide and the commented
% code.

% \begin{acks}
%   The authors would like to thank Dr. Yuhua Li for providing the
%   MATLAB code of the \textit{BEPS} method.

%   The authors would also like to thank the anonymous referees for
%   their valuable comments and helpful suggestions. The work is
%   supported by the \grantsponsor{GS501100001809}{National Natural
%     Science Foundation of
%     China}{http://dx.doi.org/10.13039/501100001809} under Grant
%   No.:~\grantnum{GS501100001809}{61273304}
%   and~\grantnum[http://www.nnsf.cn/youngscientists]{GS501100001809}{Young
%     Scientists' Support Program}.

% \end{acks}


==> section-abstract-edited.tex <==
% scratch space to consolidate my thoughts ~ Saurabh

Challenges
* Hard to train embeddings for large sparse graphs with high dimensionality (do we really have high dimensionality?)
* 

Contributions
* 

Working with sparse, high-dimensional graphs can be challenging in machine learning. Traditional ML architectures can only learn weights for a limited number of features, and even highly flexible neural networks can become overburdened if there isn't enough data. We'll discuss neural graph embeddings, used extensively in unsupervised dimensionality reduction of large graph networks. They can also be used as a transfer learning layer in other ML tasks. We'll explain our proposed architecture, which is highly scalable while keeping node types in their own distinct embedding space. Our approach involves a massively scalable architecture for distributed training in which the graph is distributed across a number of computational nodes that can fetch and update parameters of the embedding space. The parameters are served from several servers that scale with the number of parameters. We'll share our preliminary results showing training acceleration and reduced time to convergence.

Learning high quality embedding vectors for abstract entities that are far removed from the NLP space is an area of active research in the industry. Previous approaches like Word2Vec and Facebook's StarSpace system primarily focus on representing document or word embeddings, however these techniques fall short on representing more abstract entities like the merchants, customer accounts, or geospatial information from Capital One's own transactional logs. In this paper, we propose a large-scale graph embeddings framework for constructing distributed vector representations for billions of the aforementioned entities. We represent the aforementioned merchants, accounts, and zips as a relationship graph and dynamically allocate subgraphs to many different workers in a distrubted kubernetes platform. In order to train on such a large graph, we horizontally scale our system without partitioning subgraphs across worker nodes. This approach also allows each worker node to train independently from one another heavily reducing network bandwidth costs from cross-communication and boosting convergence speed due to each system training asynchronously. We quanitatively demonstrate the effectiveness of our system by tracking convergence speed and measuring link prediction accuracy across the billion-wide transactional graph. We conclude this work by discussing how high quality embeddings can positively impact downstream applications at Capital One, such as recommendation engines, fraud detection systems, and other tools.

-horizontally partitions the number of data samples across many different worker nodes that also avoids p

-system is novel for what reasons
    -one, we propose a syste

-Learn high quality embeddings for abstract entities that are far removed from the NLP space, and learn a distributed vector representation for these nodes in a large-scale graph embeddings framework.
-Draw inspiration from a variety of applications that employ large-scale graph frameworks for creating meaningful relationships between millions if not billions of different entities.
-Used link prediction accuracy to measure results; we demonstrate an increase in prediction accuracy with our large-scale distributed system
-trained on Capital One's internal transaction logs that includes data relating merchants, customer accounts, and geospatial information to learn embeddings that can represent these three entities in a meaningful manner.
-
\footnote{This is an abstract footnote}

==> section-experiments.tex <==
\section{Experiments}
Detailed description

\subsection{Dataset}

% \subsection{Results}
